Taxonomy-Aware Evaluation of Vision-Language Models

When a vision-language model (VLM) is prompted to identify an entity depicted in an image, it may answer 'I see a conifer,' rather than the specific label 'norway spruce'. This raises two issues for evaluation: First, the unconstrained generated text needs to be mapped to the evaluation label space (i.e., 'conifer'). Second, a useful classification measure should give partial credit to less-specific, but not incorrect, answers ('norway spruce' being a type of 'conifer'). To meet these requirements, we propose a framework for evaluating unconstrained text predictions, such as those generated from a vision-language model, against a taxonomy. Specifically, we propose the use of hierarchical precision and recall measures to assess the level of correctness and specificity of predictions with regard to a taxonomy. Experimentally, we first show that existing text similarity measures do not capture taxonomic similarity well. We then develop and compare different methods to map textual VLM predictions onto a taxonomy. This allows us to compute hierarchical similarity measures between the generated text and the ground truth labels. Finally, we analyze modern VLMs on fine-grained visual classification tasks based on our proposed taxonomic evaluation scheme.

==> macros.tex <==

\pdfoutput=1 

\usepackage{mathtools}
\usepackage{ellipsis}
\makeatletter
\renewcommand*{\mathellipsis}{%
  \mathinner{%
    \kern\ellipsisbeforegap%
    {\ldotp}\kern\ellipsisgap%
    {\ldotp}\kern\ellipsisgap%
    {\ldotp}\kern\ellipsisaftergap%
  }%
}
\renewcommand*{\dotsb@}{%
  \mathinner{%
    \kern\ellipsisbeforegap%
    {\cdotp}\kern\ellipsisgap%
    {\cdotp}\kern\ellipsisgap%
    {\cdotp}\kern\ellipsisaftergap%
  }%
}
\renewcommand*{\@cdots}{%
  \mathinner{%
    \kern\ellipsisbeforegap%
    {\cdotp}\kern\ellipsisgap%
    {\cdotp}\kern\ellipsisgap%
    {\cdotp}\kern\ellipsisaftergap%
  }%
}
\renewcommand*{\ellipsis@default}{%
  \ellipsis@before
  \kern\ellipsisbeforegap
  .\kern\ellipsisgap
  .\kern\ellipsisgap
  .\kern\ellipsisgap
  \ellipsis@after\relax}
\renewcommand*{\ellipsis@centered}{%
  \ellipsis@before
  \kern\ellipsisbeforegap
  .\kern\ellipsisgap
  .\kern\ellipsisgap
  .\kern\ellipsisaftergap
  \ellipsis@after\relax}
\AtBeginDocument{%
  \DeclareRobustCommand*{\dots}{%
    \ifmmode\@xp\mdots@\else\@xp\textellipsis\fi}}
\def\ellipsisgap{-.05em}
\def\ellipsisbeforegap{-.05em}
\def\ellipsisaftergap{.05em}
\makeatother

% highlighting in mathmode
\newcommand{\mathhl}[2][yellow!80]{\mathchoice%
    {\colorbox{#1}{$\displaystyle#2$}}%
    {\colorbox{#1}{$\textstyle#2$}}%
    {\colorbox{#1}{$\scriptstyle#2$}}%
    {\colorbox{#1}{$\scriptscriptstyle#2$}}}%

%\usepackage{marginnote}

\newcommand{\paroutline}[1]{\reversemarginpar\marginpar{\vspace{\baselineskip}{\scriptsize\color{ETHPurpleDark} #1}}\normalmarginpar}
%\newcommand{\paroutline}[3][false]{%
%    \ifnum\pdfstrcmp{#1}{true}=0
%        #3% Print only the second argument
%    \else
%        [\textit{\textcolor{DiverseMagenta}{#2}}] \textcolor{AccentBlue}{#3}% Print both arguments
%    \fi
%}

\usepackage[normalem]{ulem} % For underlining with squiggles
%\usepackage[dvipsnames]{xcolor}


% ETH colors
\definecolor{ETHBlue}{RGB}{33,92,175}   % blue
\definecolor{ETHGreen}{RGB}{98,115,19}      % green
\definecolor{ETHPurpleDark}{RGB}{140,10,89} % purple
\definecolor{ETHPurple}{RGB}{163,7,116} % purple
\definecolor{ETHGray}{RGB}{111,111,111} % gray
\definecolor{ETHRed}{RGB}{183,53,45}    % red
\definecolor{ETHPetrol}{RGB}{0,120,148} % green/blue
\definecolor{ETHBronze}{RGB}{142,103,19}    % bronze
\definecolor{ETHOrange}{RGB}{230, 100, 50}

\colorlet{MacroColor}{ETHPetrol}
\colorlet{MACROCOLOR}{MacroColor}

\definecolor{WildStrawberry}{rgb}{1.0, 0.26, 0.64}
\definecolor{Wisteria}{rgb}{0.79, 0.63, 0.86}
\definecolor{Olive}{rgb}{0.5, 0.5, 0.0}
\definecolor{Plum}{rgb}{0.56, 0.27, 0.52}

\renewcommand{\qedsymbol}{$\blacksquare$}

\usepackage[capitalize,noabbrev]{cleveref}
\crefname{section}{\S}{\S\S}
\crefname{table}{Tab.}{Tab.}
\crefname{figure}{Fig.}{Figs.}
\crefname{algorithm}{Alg.}{}
\crefname{equation}{Eq.}{Eq.}
\crefname{appendix}{App.}{}
\crefname{theorem}{Theorem}{}
\crefname{prop}{Proposition}{}
\crefname{definition}{Def.}{}
\crefname{cor}{Corollary}{}
\crefname{observation}{Observation}{}
\crefname{assumption}{Assumption}{}
\crefname{hyp}{Hyp.}{Hypotheses}
\crefformat{section}{\S#2#1#3}
\crefname{namedtheorem}{Hyp.}{Hypotheses}

% Theorem Environment commands
% \newtheorem{defin}{Definition}
\newtheorem{lemma}{Lemma}
\newtheorem{remark}{Remark}
\newtheorem{theorem}{Theorem}
\newtheorem{construction}{Construction}
\newtheorem{proposition}{Proposition}
\newtheorem{conjecture}{Conjecture}
\newtheorem{definition}{Definition}
\newtheorem{myexample}{Example}
\newtheorem{mytransform}{Transform}
\newtheorem{corollary}{Corollary}


% Define a command for squiggly red underline
\newcommand{\squigglyred}[1]{\textcolor{red!70!black}{\uwave{#1}}}


\newcommand{\edit}[1]{{\color{red}[#1]}}
\newcommand{\editrm}[1]{{\color{red}\st{[#1]}}}


\newcommand{\cut}[1]{{\color{black!20!red!20}#1}}
\newcommand{\fix}[1]{{\color{red}[\textbf{fix:} #1]}}
\newcommand{\draft}[1]{{\color{ETHPurpleDark} #1}}
\newcommand{\rephrase}[1]{\squigglyred{#1}}
\newcommand{\saveforcameraready}[1]{}

\newcommand{\marked}[0]{{}^{\#}}

% \newcommand{\justification}[1]{\text{\footnotesize {\color{ETHGray}(#1)}}}

\newcommand{\justification}[1]{%
    \refstepcounter{equation}%
    \tag{\theequation \textcolor{black!50}{, \footnotesize{#1}}}
}

\newcommand{\prooftext}[1]{\text{\color{black!50}#1}}
\newcommand{\proofExplain}[1]{\text{\scriptsize\color{black!50}[#1]}}
\newcommand{\proofExplainLong}[2][1.5in]{%
{\scriptsize\color{black!50}%
\left[\begin{minipage}[c]{#1}%
#2%
\end{minipage}\right]}%
}

\newcommand{\defn}[1]{\textbf{#1}}
%\newcommand{\defeq}{\mathrel{\raisebox{-0.3ex}{\overset{\raisebox{-0.25ex}{\textnormal{\tiny def}}}{=}}}}
\newcommand{\defeq}{\mathrel{\overset{\raisebox{-0.25ex}{\textnormal{\tiny def}}}{=}}}

\newcommand{\card}[1]{\left|#1\right|}

\newcommand{\simIID}[0]{\mathrel{\overset{{\scriptsize\text{i.i.d.}}}{\sim}}}

%\newcommand{\defeq}{\stackrel{\text{def}}{=}}
%\newcommand{\defpropto}{\mathrel{\stackrel{\textnormal{\tiny def}}{\propto}}}

\newcommand{\set}[1]{\left\{ #1 \right\}}

\newcommand{\indicator}[1]{\mathbbm{1}\mleft\{#1\mright\}}

\newcommand{\idfun}{\mymacro{\text{Id}}}

\newcommand{\bigo}{{\mymacro{ \mathcal{O}}}}
\newcommand{\bigO}[1]{{\mymacro{ \bigo\mleft(#1\mright)}}}
\newcommand{\bigOmega}[1]{{\mymacro{ \Omega\mleft(#1\mright)}}}

\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}

\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}


\newcommand{\exactagg}{{\mymacro{\textsc{Exact}}}}
\newcommand{\sumagg}{{\mymacro{\textsc{Sum}}}}
%\newcommand{\prodagg}{{\mymacro{\textsc{Prod}}}}
\newcommand{\meanagg}{{\mymacro{\textsc{Mean}}}}
\newcommand{\firstagg}{{\mymacro{\textsc{First}}}}
\newcommand{\surprisal}{{\mymacro{h}}}
\newcommand{\entropy}{\mymacro{\mathrm{H}}}

\newcommand{\setX}{{\mymacro{\mathcal{X}}}}
\newcommand{\setY}{{\mymacro{\mathcal{Y}}}}
\newcommand{\setZ}{{\mymacro{\mathcal{Z}}}}
\newcommand{\elemx}{{\mymacro{x}}}
\newcommand{\elemy}{{\mymacro{y}}}
\newcommand{\elemz}{{\mymacro{z}}}
\newcommand{\mapf}{{\mymacro{f}}}
\newcommand{\mapg}{{\mymacro{g}}}

\newcommand{\cover}{{\mymacro{\mathcal{C}}}}
\newcommand{\leakage}{\mymacro{\lambda}}


\newcommand{\abstractalphabet}{{\mymacro{ \Gamma}}}
\newcommand{\abstractStrings}{{\mymacro{ \Gamma^*}}}
\newcommand{\abstractstring}{{\mymacro{ \boldsymbol{\gamma}}}}
\newcommand{\abstractsymbol}{{\mymacro{\gamma}}}
\newcommand{\abstracteosalphabet}{{\mymacro{\overline{\Gamma}}}}

\newcommand{\wordalphabet}{{\mymacro{\Omega}}}
\newcommand{\eoswordalphabet}{{\mymacro{\overline{\wordalphabet}}}}
\newcommand{\prewords}{{\mymacro{\widetilde{\Omega}}}}
\newcommand{\word}{{\mymacro{w}}}
\newcommand{\wordseq}{{\mymacro{\boldsymbol{w}}}}



\newcommand{\tokAlphabetwhite}{\tokAlphabet_1}
\newcommand{\tokAlphabetnowhite}{\tokAlphabet_2}

\newcommand{\kleene}[1]{#1^*}
\newcommand{\kleeneplus}[1]{#1^+}

%\newcommand{\textexample}[1]{{\mymacro{ \fontfamily{ppl}\selectfont \text{``#1''}}}}

\newcommand{\bos}{{\mymacro{\textsc{bos}}}}
\newcommand{\eos}{{\mymacro{\textsc{eos}}}}


\newcommand{\normconstant}{\mymacro{Z}}
\newcommand{\normconstanttwo}{\mymacro{Y}}


\DeclareTextCommandDefault{\textvisiblespace}{%
  \mbox{\kern.06em\vrule \@height.3ex}%
  \vbox{\hrule \@width.3em}%
  \hbox{\vrule \@height.3ex}}


% \newcommand{\ptext}{\mymacro{p}}
% \newcommand{\idalpha}{\mymacro{\textnormal{id}_{\charStrings}}}
% \newcommand{\vdot}{{\mymacro \shortmid}}
% \newcommand{\adot}{\mymacro \cdot}
% \newcommand{\lexicon}{\mymacro \Gamma}
% \newcommand{\spell}{\mymacro \lambda}
% \newcommand{\rLM}{\mymacro r}
% \newcommand{\qSM}{\mymacro q_{\textsc{sm}}}

\newcommand{\pcontext}{\mymacro{c_{\charAlphabet}}}

% \newcommand{\sentence}{\mymacro{\boldsymbol{\gamma}}}
% \newcommand{\word}{\mymacro{\gamma}}
%\newcommand{\sentence}{\texts}
% \newcommand{\prerlm}{\mymacro{\pi_{\rLM}}}
% \newcommand{\preqlm}{\mymacro{\pi_{\qLM}}}

\renewcommand{\c}[0]{{\cdot}}

\definecolor{CharacterColor}{RGB}{98,115,19}
\definecolor{TokenColor}{RGB}{140,10,89} 

% used in token probability plots
\newcommand{\probbar}[1]{%
\makebox[1cm][r]{\rule{#1\linewidth/4}{5pt} {\scriptsize\color{black!50} (#1)}} 
}

% Custom truncated box
\newcommand{\custombox}[1]{%
    \begin{tikzpicture}[baseline={(current bounding box.center)}]
        % Define the node with no borders
        \node[anchor=north west] (box) at (0,0) {#1};
        
        % Draw only the top, left, and right sides of the box
        \draw[thin, black!25] (box.south west) -- (box.north west) -- (box.north east) -- (box.south east);
        
        % Draw the wavy truncation line at the bottom
        \draw[thin, black!25] 
            (box.south west) .. controls +(0.3cm,0.15cm) and +(-0.3cm,-0.15cm) .. ++(0.6cm,0) 
            .. controls +(0.3cm,0.15cm) and +(-0.3cm,-0.15cm) .. ++(0.6cm,0)
            .. controls +(0.3cm,0.15cm) and +(-0.3cm,-0.15cm) .. ++(0.6cm,0)
            .. controls +(0.3cm,0.15cm) and +(-0.3cm,-0.15cm) .. (box.south east); % Smooth wavy line
    \end{tikzpicture}%
}

%\newcommand{\tokenfont}[2][]{\ensuremath{\underset{{\scriptsize\texttt{#1}}}{{\color{TokenColor}\scriptsize\texttt{#2}}}}}
\newcommand{\ttttokenfont}[2][]{%
\ensuremath{\stackrel{{\scriptsize\color{TokenColor}\texttt{#2}}}{{\color{black!50}\scriptsize\texttt{#1}}}}%
}
% Improved tokenfont command with raisebox
\newcommand{\tokenfont}[2][]{%
    \ensuremath{%
        \stackrel{\raisebox{-0.5ex}{{\color{TokenColor}\scriptsize\texttt{#2}}}}%
        {\raisebox{-0.5ex}{{\scriptsize\color{black!50}\texttt{\strut#1}}}}%
    }%
}
% \newcommand{\tokenfont}[2][]{\ensuremath{%
% \genfrac{}{}{0pt}{}%
% {{\color{TokenColor}\texttt{#2}}}%
% {{\scriptsize\texttt{#1}}}%
% }}
\newcommand{\charfont}[1]{{\color{CharacterColor}\texttt{\small#1}}}

\newcommand{\tokmodel}{\mymacro{\mathcal{T}}}
\newcommand{\tokenizer}{\ensuremath{{\color{TokenColor}\tau}}\xspace}
\newcommand{\cotokenizer}{\ensuremath{{\color{CharacterColor}\kappa}}\xspace}

\newcommand{\tokenizerBPE}[0]{\ensuremath{\tokenizer_{{\color{TokenColor}\text{BPE}}}}\xspace}
\newcommand{\cotokenizerBPE}[0]{\ensuremath{\cotokenizer_{{\color{CharacterColor}\text{BPE}}}}\xspace}
\newcommand{\D}[0]{{\color{TokenColor}D}}
\newcommand{\notD}[0]{{\color{TokenColor}\overline{D}}}
\newcommand{\preD}[0]{{\color{TokenColor}\prefixLanguageOp{D}}}

\newcommand{\token}{{\color{TokenColor}\delta}}
\newcommand{\tokseq}{\ensuremath{{\color{TokenColor}\boldsymbol{\delta}}}\xspace}
\newcommand{\tokStrings}[0]{{\color{TokenColor}\kleene{\tokAlphabet}}}
\newcommand{\tokAlphabet}{{\color{TokenColor}\Delta}}

\newcommand{\chars}{{\color{CharacterColor}\sigma}}
\newcommand{\charseq}{{\color{CharacterColor}\boldsymbol{\sigma}}}
\newcommand{\charseqTarget}{{\color{CharacterColor}\boldsymbol{\widehat{\sigma}}}}
\newcommand{\charsTarget}{{\color{CharacterColor}\widehat{\sigma}}}
\newcommand{\charAlphabet}{{\color{CharacterColor}\Sigma}}
\newcommand{\charStrings}[0]{{\color{CharacterColor}\kleene{\charAlphabet}}}

\newcommand{\ptokens}{\mymacro{p_{\tokAlphabet}}}
\newcommand{\pchars}{\mymacro{p_{\charAlphabet}}}
\newcommand{\pabstract}{\mymacro{p_{\abstractalphabet}}}

\newcommand{\prefixLanguageOp}[1]{\overrightarrow{#1}}
\newcommand{\prefixClosure}[1]{\prefixLanguageOp{#1}}
\newcommand{\prefixAbstract}{\mymacro{\prefixLanguageOp{\pabstract}}}
\newcommand{\prefixTokens}{{\mymacro{\prefixLanguageOp{\ptokens}}}}
\newcommand{\prefixChars}{{\mymacro{\prefixLanguageOp{\pchars}}}}

%\newcommand{\modelchars}[0]{\mymacro{\widehat{\pchars}}}
%\newcommand{\modeltokens}[0]{\mymacro{\widehat{\ptokens}}}

%\newcommand{\empiricaltokens}{\mymacro{\widehat{p}_{\tokAlphabet}}}
%\newcommand{\empiricalcontexttokens}{\mymacro{\widehat{c}_{\tokAlphabet}}}

%\newcommand{\canonmodelchars}{\mymacro{\overline{q}_{\charAlphabet}}}
%\newcommand{\legal}[0]{\mathrm{legal}}
%\newcommand{\prefixLegal}[0]{\prefixLanguageOp{\mathrm{legal}}}
%\newcommand{\approxpchars}{{\mymacro{\overline{p}_{\charAlphabet}}}}

\renewcommand{\Pr}[2][]{\mathop{\mathrm{Pr}}_{#1}\mleft[#2\mright]}






% --- notation

\DeclareRobustCommand{\bbone}{\text{\usefont{U}{bbold}{m}{n}1}}
\DeclareMathOperator{\EX}{\mathbb{E}}

